Test them all, is it worth it? Assessing configuration sampling on the JHipster Web development stack

Many approaches for testing configurable software systems start from the same assumption: it is impossible to test all configurations. This motivated the definition of variability-aware abstractions and sampling techniques to cope with large configuration spaces. Yet, there is no theoretical barrier that prevents the exhaustive testing of all configurations by simply enumerating them, if the effort required to do so remains acceptable. Not only this: we believe there is lots to be learned by systematically and exhaustively testing a configurable system. In this case study, we report on the first ever endeavour to test all possible configurations of an industry-strength, open source configurable software system, JHipster, a popular code generator for web applications. We built a testing scaffold for the 26,000+ configurations of JHipster using a cluster of 80 machines during 4 nights for a total of 4,376 hours (182 days) CPU time. We find that 35.70% configurations fail and we identify the feature interactions that cause the errors. We show that sampling strategies (like dissimilarity and 2-wise): (1) are more effective to find faults than the 12 default configurations used in the JHipster continuous integration; (2) can be too costly and exceed the available testing budget. We cross this quantitative analysis with the qualitative assessment of JHipster's lead developers.

==> parts_related.tex <==
\section{Related Work}
\label{sec:related}

The difficulty to assess all the possible configurations in the general case lead to the development of various sampling techniques, differing by their coverage criteria (e.g., pair-wise \cite{yilmaz2006covering, Cohen2008,Perrouin2011} or dissimilarity amongst configurations \cite{Henard2014a}), use of exact algorithms \cite{Johansen2016,Hervieu2011}, or metaheuristics \cite{garvin2011evaluating,Sayyad2013c,Parejo2016,Henard2014a}. 

\subsection{Comparison of Sampling Strategies} 

Perrouin \etal \cite{Perrouin2011} compared two exact approaches on five feature models of the SPLOT repository w.r.t to performance of t-wise generation and configuration diversity. Hervieu \etal \cite{Hervieu2011} also used models from the SPLOT repository to produce a small number of configurations. Empirical investigations were pursued on larger models (1,000 features and above) notably on OS kernels (e.g., \cite{Henard2014a,Johansen2012}) demonstrating the relevance of metaheuristics for large sampling tasks \cite{Henard2015,Ochoa:2017:SSP:3023956.3023959}.  However, these comparisons were performed at the model level (there was no product associated to these models) using artificial faults. 

Several authors considered sampling on actual systems, thus dealing with real faults. Johansen \etal \cite{DBLP:conf/models/JohansenHFES12} extended SPLCAT by adding weights on sub-product lines and apply their approach to the Eclipse IDE and to TOMRA, an industrial product line. Steffens \etal \cite{Oster2011} applied the Moso-Polite pairwise tool on an electronic module allowing 432 configurations to derive metrics regarding the test reduction effort. Additionally, they also exhibited a few cases where an higher interaction strength was required (3-wise). Sanchez \etal \cite{Sanchez:2014:DFC:2556624.2556638} modelled a subset of the Drupal framework and (manually) examined how faults (extracted from the Drupal's issue tracking system) were related to feature interactions: Amongst 390 faults, 11 were related to 2-wise interactions, 1 to 3-wise interactions, and the rest was related to single features. A further analysis on this case revealed that with respect to 3,392 faults, 160 were related to up to 4-wise interactions \cite{Sanchez2017}. Medeiros \etal \cite{MKRGA:ICSE16} compared 10 sampling algorithms on a corpus of existing configurations faults taken from a large set of configurable systems. The authors found that 2-wise interactions covered a large subset of faults (as it is commonly assumed) but also made the case for higher-interaction strengths (seven in their study) and that sampling algorithms such as most-enabled-disabled are most efficient in that case. Our study adds more empirical evidence on the fact that higher-interaction is desirable to find all bugs. %However, in our case the most-enabled-disabled strategy did select a high number of sample which greatly reduced its efficiency.  

Despite the number of empirical investigations (e.g., \cite{ganesan2007comparing,qu2008configuration}) and surveys (e.g., \cite{Engstrom2011,DBLP:journals/csur/ThumAKSS14,DaMotaSilveiraNeto2011}) to compare such approaches, many focused on subsets to make the analyses tractable. Being able to execute all configurations led us to consider actual failures and collect a ground truth. It helps to gather insights for better understanding the interactions in large configuration spaces ~\cite{MWKTS:ASE16,yilmaz2006covering}.  

%\subsection{Testing in the Wild} 
\subsection{Testing at Scale} 

Greiler \etal \cite{GreilerConfessions} investigated how developers tested their plug-ins in the Eclipse framework.  The prevalent technique used was unit testing of individual plug-ins without any systematic approach to handle combination with other plugins. Interviewed people complained about the difficulty to set up a proper integration environment, long execution times (few minutes), and lack of best practices. In the case of JHipster, we reported on similar difficulties with the testing environment. Furthermore, execution time prevailed on the testing budget: it took 1h30 to build and test 12 configurations. However, the JHipster team is eager to try quicker ways for building of configurations and for the last release (4.0), they extended the budget to 19 configurations.   

A case study at Google reported a large corpus of builds and build errors mainly focusing on static compilation problems~\cite{Seo:2014:PBE:2568225.2568255}.
Beller \etal \cite{Beller:2017:OMT:3104188.3104232} performed an analysis of builds with Travis CI on top of GitHub. One interesting insight is that about 10\% of builds show different behaviour when different environments are used. It is related to our endeavour to build the "good" distributed environment for testing JHipster at scale.  





